Bayesian Persuasion for Containing SIS Epidemics with Asymptomatic Infection

We investigate the strategic behavior of a large population of agents who decide whether to adopt a costly partially effective protection or remain unprotected against the susceptible-infected-susceptible epidemic. In contrast with most prior works on epidemic games, we assume that the agents are not aware of their true infection status while making decisions. We adopt the Bayesian persuasion framework where the agents receive a noisy signal regarding their true infection status, and maximize their expected utility computed using the posterior probability of being infected conditioned on the received signal. We characterize the stationary Nash equilibrium of this setting under suitable assumptions, and identify conditions under which partial information disclosure leads to a smaller proportion of infected individuals at the equilibrium compared to full information disclosure, and vice versa.

==> legacy.tex <==
%\begin{remark}
%\um{It is interesting to note that the value of the infection state equilibrium point $\yint = \frac{C_{\Pt}}{(1-\alpha) L \beta_{\Pt}}$ remains unchanged with any variation of $\mu_{S}$. However, the upper bound, which determines convergence to the investigated equilibrium point, is dictated by $\mu_{S}$, i.e., is monotonically increasing in $\mu_{S}$. In this case as well we do not benefit from the signalling scheme as the infection state equilibria in both, full and partial information disclosure, are equal.}
%\end{remark}
%\begin{remark}
%    \um{This is the most significant proposition as far as reducing infected fraction is concerned. Need to add a detailed discussion.}
%\end{remark}

%Suppose $\mu^{\max}_{\St} > 0$ and $\mu_{\St} < \mu^{\max}_{\St}$. In this case, $g(0,\mu_{\St}) < 0 \iff \Delta U[\Itb](1,0;\mu_{\St}) < 0$, which implies $\zibar=0$ can not be SNE. In addition, it follows from Proposition \ref{prop:unstable} that
%$$ g(z^\star_{\Itb},\mu_{\St}) \leq 0 \implies \Delta U [\Stb](1,z_{\Itb};\mu_{\St}) < 0.$$
%We now have two possibilities. 
%\begin{itemize}
%    \item Case 1: $g(1,\mu_{\St}) \leq 0 \implies g(z_{\Itb},\mu_{\St}) < 0$ for all $z_{\Itb} \in [0,1]$. 
%    \item Case 2: $g(1,\mu_{\St}) > 0$ which implies there exists unique $z^\star_{\Itb} \in (0,1)$ such that $g(z^\star_{\Itb},\mu_{\St})=0$. 
%\end{itemize}

%We define the following quantity. 
%\begin{align}\label{eq:def_mus_max}
%    \mu^{\min}_{\St} := 1 - \frac{(\betau - \gamma) (C_{\Ut} - C_{\Pt})}{\gamma (C_{\Pt} - (1-\alpha) L (\beta_{\Ut} -\gamma))}. 
%\end{align}
%We now consider the first case below. 

%We define
%Combination of values from Table \ref{tab:common} and choosing $C_{\Pt} = 1.5$ yields $y^*_{\Pt} = 0.111 > \yint = 0.068$. As per equilibrium characterization in Theorem \ref{theorem:main}, the condition $y^*_{\Pt} > \yint$ leads to convergence of the states to theoretically computed SNE $(y^*_{\Pt}, 0, 0)$, which is in accordance with the top left plot of Figure \ref{fig:Plot}. Similarly, conditions pertaining to rest of the SNEs derived from Theorem \ref{theorem:main} and the values obtained from Table \ref{tab:common} and \ref{tab:specific} can be used to verify the other convergences. 
%begin{remark}
%The above equilibrium does not arise in the FID setting. Discuss why it arises in this case and what is its interpretation. \um{The first condition is sufficient to guarantee that $z^\star_{\Stb}=1$. If the second and third conditions are not true, then we cannot have $z^\star_{\Itb}=1$. However, it is possible to have equilibria with $z^\star_{\Itb}<1$.}
%\end{remark}

%Scrutinizing the applications, routing games and traffic congestion is a popular area that exploits Bayesian persuasion, \cite{ferguson2022avoiding, tavafoghi2019strategic, verbree2021inferring, wu2021value}. Congestion games involves players who are uncertain about the states in a transportation network, and strategical information design addresses this gap of partial information. In \cite{acemoglu2018informational}, the authors have introduced Informational Braess' Paradox and answered the fundamental question of whether providing additional information worsens the situation. Apart from traffic system, internet routing with incomplete knowledge has been studied in \cite{seaton2023competitive}. Some other fields engaging information design range from implementing electricity demand-response programs \cite{aid2023signalling}; security enhancement \cite{farhadi2018static}; contracting experimental research \cite{yoder2022designing}; government controlling media \cite{gehlbach2014government}; tests and trials for drug approval \cite{kolotilin2015experimental}. Two works that throw light upon the diversity captured by Bayesian persuasion model are \cite{kamenica2019bayesian}, and \cite{bergemann2019information}.

%The only work within an epidemiological framework that examines Bayesian persuasion for curbing spread of infection is \cite{pathak2022scalable}. To the best of our knowledge, ours is the first work that integrates an epidemic model to Bayesian persuasion, and analyses the stability of the existing equilibrium points. Our work differs from \cite{pathak2022scalable} mainly in terms of the model. We consider a well-known infection spreading process, in which the dynamics is dictated by a modified version of SIS epidemic model, whereas, in \cite{pathak2022scalable} the authors have considered a network framework represented by a graph structure (without specific reference to any epidemic model). As a result, we consider a very large homogeneous population, in which the agents receiving a particular signal have the same belief, while Pathak et al. focus on the effect of connections between nodes. The game-setting in our paper involves a discrete action set of adopting protection, or remaining unprotected for the agents, who themselves do not know their true states. Protection is partially effective and comes at a cost. The individuals possessing Bayesian rationality compute their posterior based on the prior and partial information disclosed under the signalling scheme. We prove analytically that under certain conditions, there is a successful curtailment of infection level at equilibrium, in comparison to the case when the individuals have full information of their states.

%Outbreak of an infectious disease results in far-reaching monetary and life losses. Thereby, under such situations, effective reduction of epidemic spread undisputedly becomes the main objective of governments. Such spreading processes are predominantly governed by human interactions that take place. Spread of the infectious disease is shaped by human behaviour, which in turn changes the infection level, as studied in \cite{ferguson2007capturing}, \cite{chen2013behavioral}. Prior works include modeling the infection spread within a game-theoretic framework. Instead of individual agents, when actions chosen by sub-populations as a whole are of interest, modeling through mean-field games and study of herd behaviour is pertinent (see \cite{liu2022herd}, \cite{liu2022understanding}). Control of epidemic spread through mean-field games model has also been investigated in \cite{lee2020controlling}. Epidemic containment game on networks has been studied in \cite{saha2014equilibria}, \cite{xu2018extended}, \cite{hu2023stackelberg}. \cite{huang2022game} includes a comprehensive review of strategic decision-making by individuals. At the onset of an infection, when there exists no medication/vaccination as a remedy, policy-makers heavily depend on non-pharmaceutical interventions (NPIs) to contain the epidemic spread (see \cite{angulo2021simple}, \cite{kantner2020beyond}). NPIs vary from using masks, PPE kits, sanitizers etc. to maintaining social distance, and implementation of lockdowns and quarantining zones. However, the tendency of individuals to adopt protection and follow isolation rules is determined by the rewards and incentives they receive in due process.  

%Motivated by the recent COVID-19 pandemic, in this paper we analyse an SIS epidemic model, subjected to a signalling scheme. By incorporating a game-setting involving actions of adopting protection or remaining unprotected, as in \cite{satapathi2022epidemic}, we have deviated from the standard SIS model. Most of the previous works on epidemics analyse human behavioural aspects and disease propagation taking into account that the agents have full information regarding their states. However, in absence of symptoms, or because of the existence of same symptoms due to multiple diseases, accurate information of an individual's state may not be available with her. As a result, she receives an estimate of her true state from external environment. Analysing the impact of partial information of agents regarding their state which strongly dictates epidemic propagation has been largely unexplored. We examine this gap by incorporating a signalling scheme, which gives the agents some information about their states. We further model our agents as \emph{Bayesian decision-makers} to investigate the effect of signals (providing partial information), that encourage agents to choose different actions which in turn changes infection level, compared to the case when agents have precise information of their states. We answer the following questions in this paper. What are the stable equilibrium points that exist under the signalling provision, and what are the parameter regimes in which they are stable? Does the infection level increase, decrease, or remain the same in partial information disclosure, compared to the full information availability case? Is the amount of information conveyed to the agents capable of controlling the infection level at equilibrium? Before proceeding with the problem and detailed analyses, we discuss some previous works in the area of Bayesian persuasion.

%\subsection{Prior Works on Bayesian Persuasion}

%Selective information disclosure in real-world socio-economic situations is a popular technique to persuade an individual to choose an action that benefits the information sender. %For example, information design can be used by a seller to strategically make certain information available to the buyers, who in turn choose actions based on limited information that benefits the buyer.
%\cite{kamenica2011bayesian} deals with a setting of judicial proceeding, in which the prosecutor uses Bayesian persuasion to increase probability of conviction of an accused by a rational judge. Kamenica et al. analyse a two-player game in which information sender enjoys an advantage by transmitting partial information to the receiver. %Previous studies have analysed how \emph{cheap talk} is persuasive, see \cite{chakraborty2010persuasion}. In \cite{sagiev2020bayesian} the author has integrated cheap talk and Bayesian persuasion in a single model, and proves the condition under which Bayesian persuasion aids in making cheap talk more informative. %In this model, there also exists a mediator, who provides her own understanding of information in order to convince the receiver. A detailed study beyond the traditional sender-receiver game-setting by including uninformed mediators, and their contribution to Bayesian persuasion is found in \cite{arieli2022bayesian}.
%The concept of multiple receivers in Bayesian persuasion is introduced in \cite{wang2013bayesian}. Existence of multiple receivers is highly relevant in real-life investigation procedures, like testing of new medicines. The author compares public persuasion, in which all receivers have a common observation, with private persuasion (receivers get separate observations). An extension of multiple receiver in Bayesian persuasion is \cite{castiglioni2021multi}, in which under a full-information feedback setting the sender is unaware of the receivers' utilities. The authors examine an online learning technique based on no-regret algorithm for the sender. Unlike the above mentioned works, \cite{matyskova2023bayesian}, and \cite{nguyen2021bayesian} departs from the classical Bayesian model by introducing costs in information transmission. %Similar to multiple receivers, the notion of multiple senders and a single receiver has been introduced in \cite{gentzkow2017bayesian}, in which each sender with no \emph{ex ante} private information privately observes her signal realization. %Based on certain assumptions, the authors show that increasing the number of senders do not decrease the amount of information. A further extension to \cite{gentzkow2017bayesian} is \cite{li2018bayesian}, in which the authors prove that violation of any of the assumptions mentioned in the former work results in loss of information on including additional senders.

%In the former, the authors analyse changes in the players' well-being with a reduction in receiver's cost of information. Whereas, in the latter work the authors deal with a \emph{lying cost}, which reduces the aggregate utility of the sender. 
%Ricardo et al. in \cite{alonso2016bayesian} have considered a game-setting involving a politician and a bureaucrat, such that each holds a different prior. This dilutes the assumption of both sender and receiver with a homogeneous prior before the sender observes the signal, and decides to send information. 
%Rest of the paper unfolds as follows. In Section \ref{sec:strategic_protection} we have introduced the partially protected SIS epidemic model and the notion of partial information disclosure under faulty signalling scheme. It also includes the instantaneous rewards that individuals obtain on receiving a certain signal, based on their chosen actions. Section \ref{sec:eq_char} deals with the main contribution, i.e., characterization of the stationary Nash equilibrium under full, and partial information disclosure. In Section \ref{sec:num_result} we have included some numerical simulations, which illustrate some of the main results previously stated.
%Scrutinizing the applications, routing games and traffic congestion is a popular area that exploits Bayesian persuasion, \cite{ferguson2022avoiding, tavafoghi2019strategic, verbree2021inferring, wu2021value}. Congestion games involves players who are uncertain about the states in a transportation network, and strategical information design addresses this gap of partial information. In \cite{acemoglu2018informational}, the authors have introduced Informational Braess' Paradox and answered the fundamental question of whether providing additional information worsens the situation. Apart from traffic system, internet routing with incomplete knowledge has been studied in \cite{seaton2023competitive}. Some other fields engaging information design range from implementing electricity demand-response programs \cite{aid2023signalling}; security enhancement \cite{farhadi2018static}; contracting experimental research \cite{yoder2022designing}; government controlling media \cite{gehlbach2014government}; tests and trials for drug approval \cite{kolotilin2015experimental}. Two works that throw light upon the diversity captured by Bayesian persuasion model are \cite{kamenica2019bayesian}, and \cite{bergemann2019information}.

%It is seen that for a lower value of $\mu_{S}$ the infection level is lower as compared to its higher value. Then it follows from numerical inference that the policy-maker will be successful in maximum reduction of infection level as $\mu_{S} \rightarrow 0$. 

% To elaborate more on this, recall that $\mu_{S} = \mathbb{P}[x = \Stb | \St]$ is a quantity known to all players in our game-setting. In real-life epidemic-based situation, an individual attempts to gather some relevant information about her state, and accordingly calculates her belief. Thereby, the policy-maker makes certain information available to the agents through the signalling scheme. As $\mu_{S} \rightarrow 0$, an individual is aware of the faulty nature of signals through the known $\mu_{S}$. Accordingly, the agents may simply assume the other state (opposite to the signal they receive) as their true state. On the other hand as a more ground-level problem, agents might lose trust on the signalling arrangement, and refuse to even avail the provision to gain insights on their states. To avoid this scenario, value of $\mu_{S}$ should be as close to $1$ as possible in order to motivate individuals to opt for the scheme. This gives rise to the following problem: what should be the optimal value of $\mu_{S}$? We have analytically proved and numerically shown that within a certain parametric range the policy-maker is able to reduce infection level by not disclosing true information, but how much information should be disclosed by her? There is a trade-off between reducing equilibrium infection level and trust deficit created by not disclosing full information. As a future work/In the next section we introduce a cost that the policy-maker incurs on reducing $\mu_{S}$, i.e., the signalling scheme is costly. Naturally, this cost is dependent on $\mu_{S}$, implying lower the information disclosed, more is the penalty that policy-maker pays (primarily, the cost captures loss due to breach of trust by faulty signalling scheme). This provides an answer to the pertinent question of what is the optimal amount of information that should be revealed. 




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \section{PARTIAL VS. FULL INFORMATION DISCLOSURE}

% In this section we discuss the advantage of partial information disclosure as compared to full information disclosure. As we have assumed $\mu_I = 1$ (full information is transmitted to infected agents), i.e., all infected agents receiving infected signal are infected, the scheme of partial information affects the agents receiving susceptible signal. For the rest of our discussion in this section we assume $C_{\texttt{P}} < C_{\texttt{U}}$. In case of full information availability, we have $z_{\texttt{I}} = 0$, i.e., all infected agents adopt protection. Similarly, a susceptible agent knows its true state and chooses its action which gives a higher reward. In case of partial information disclosure, infected agents are aware of their true states. Therefore, $z_{\bar{\texttt{I}}} = z_{\texttt{I}} = 0$. However, when an agent receives a signal of being susceptible, it assumes itself to be susceptible with a certain belief. As a result it chooses an action based on its belief, which depends on its prior and $\mu_S$. Clearly, it will have a belief of itself being infected $\pi^+[\texttt{I} | \bar{\texttt{S}}] \in (0, 1)$ for $\mu_S \in (0, 1)$. Thus, $z_{\bar{\texttt{S}}} = 1$ in reality means $z_{\texttt{S}} < 1$. %\um{I have to add more}
% \\We illustrate the following by a numerical simulation. The parameters chosen for simulation purpose are given below.

% \begin{center}
% \begin{tabular}{|c | c | c | c | c | c | c | c |} 
%  \hline
%  $\alpha$ & $\beta_\texttt{P}$ & $\beta_\texttt{U}$ & $\gamma$ & $C_{\texttt{P}}$ & $C_{\texttt{U}}$ & L & $y(0)$\\ [0.5ex] 
%  \hline
%  0.2 & 0.15 & 0.3 & 0.02 & 6 & 8 & 80 & 0.1\\ \hline
% \end{tabular}
% \end{center}

% \begin{figure}[h!]
% \centering
%   \subfigure{\includegraphics[width=0.45 \linewidth]{Figures/I_levelnew.pdf}}
%   \subfigure{\includegraphics[width=0.465 \linewidth]{Figures/z.pdf}}
%   \caption{Infection state trajectory (left) and fraction of susceptible sub-population remaining unprotected (right) for different values of $\mu_{S}$.}
%   \label{figure:pid_vs_fid}
% \end{figure}
% From Figure \ref{figure:pid_vs_fid} it is clear that when $\mu_{S}$ is reduced from $1$ to $0.7$, the fraction of 
% unprotected agents receiving a signal of being susceptible decreases as more of such agents begin to adopt protection. Due to the higher fraction of sub-population adopting protection, the fall in the infection level at equilibrium is observed. This numerical result gives compelling insight that incomplete information can lead to a decrease in infection level, given the agents follow Bayesian rationality.

% \subsection{Infection Level Analyses at Equilibrium}

% In this section we compare the equilibrium infection levels obtained in both cases, and analytically derive conditions under which partial information disclosure is beneficial leading to lower infection. In case of full information disclosure, for any general fractions at equilibrium $z^*_{\texttt{S}}, z^*_{\texttt{I}}$, we have $z^*_{\texttt{S}} = z^*_{\bar{\texttt{S}}}$ and $z^*_{\texttt{I}} = z^*_{\bar{\texttt{I}}}$, as $\mu_{S} = \mu_{I} = 1$. Then, the fraction of infected sub-population at equilibrium is given by $y^*_{\mathtt{fid}} = 1 - \frac{\gamma}{(\beta_{\texttt{P}} (1 - z^*_{\bar{\texttt{I}}}) + \beta_{\texttt{U}} z^*_{\bar{\texttt{I}}}) (\alpha + (1 - \alpha) z^*_{\bar{\texttt{S}}})}$. Similarly, in partial information case with $0 < \mu_{S} < 1$ following are obtained: $z^*_{\texttt{S}} = z^*_{\bar{\texttt{S}}} \mu_{S} + z^*_{\bar{\texttt{I}}} (1 - \mu_{S})$, $z^*_{\texttt{I}} = z^*_{\bar{\texttt{I}}}$, and $y^*_{\mathtt{pid}} = 1 - \frac{\gamma}{(\beta_{\texttt{P}} (1 - z^*_{\bar{\texttt{I}}}) + \beta_{\texttt{U}} z^*_{\bar{\texttt{I}}}) (\alpha + (1 - \alpha) (z^*_{\bar{\texttt{S}}} \mu_{S} +  z^*_{\bar{\texttt{I}}} (1 -\mu_{S})))}$. Clearly, partial information disclosure is advantageous when $y^*_{\mathtt{pid}} < y^*_{\mathtt{fid}} \implies z^*_{\bar{\texttt{S}}} \mu_{S} +  z^*_{\bar{\texttt{I}}} (1 -\mu_{S}) < z^*_{\bar{\texttt{S}}}$ which on simplification yields $z^*_{\bar{\texttt{S}}} > z^*_{\bar{\texttt{I}}}$. We now investigate the combinations of $z^*_{\bar{\texttt{S}}}, z^*_{\bar{\texttt{I}}}$ which satisfy the above relation. In aggregate, there are four combinations for which above relation holds. 
% \begin{itemize}
%     \item[\textbf{(1)}] $z^*_{\bar{\texttt{S}}} = 1$, $z^*_{\bar{\texttt{I}}} = 0$;
%     \item[\textbf{(2)}] $z^*_{\bar{\texttt{S}}} = z^\dagger_{\bar{\texttt{S}}}$, $z^*_{\bar{\texttt{I}}} = 0$;
%     \item[\textbf{(3)}] $z^*_{\bar{\texttt{S}}} = 1$, $z^*_{\bar{\texttt{I}}} =  z^\dagger_{\bar{\texttt{I}}}$;
%     \item[\textbf{(4)}] $z^*_{\bar{\texttt{S}}} = z^\dagger_{\bar{\texttt{S}}}$, $z^*_{\bar{\texttt{I}}} = z^\dagger_{\bar{\texttt{I}}}$,
%\end{itemize}

\begin{proposition}
    $(1-\frac{\gamma}{\betau},1,1)$ is a SNE if and only if 
    \begin{align*}
        & 1 - \frac{\gamma}{\betau} < \frac{C_{\Pt}}{L(1-\alpha)\betau}, \quad \mu_{\St} < \mu^{\min}_{\St}, \text{and} \quad \mu^{\min}_{\St} > 0.
        %\\ & \frac{(\betau - \gamma) (C_{\Ut} - C_{\Pt})}{\gamma (C_{\Pt} - (1-\alpha) L (\beta_{\Ut} -\gamma))} < 1, \quad \text{and}
        %\\ & 1-\mu_{\St} \geq \frac{(\betau - \gamma) (C_{\Ut} - C_{\Pt})}{\gamma (C_{\Pt} - (1-\alpha) L (\beta_{\Ut} -\gamma))}. 
    \end{align*}   
    \label{prop:gamma_betau}
\end{proposition}
\begin{proof}
From Proposition \ref{prop:unstable}, it follows that $z^\star_{\Itb} = 1 \implies z^\star_{\Stb} = 1$. In addition, $y^\star(1,1;\mu_{\St}) = 1-\frac{\gamma}{\betau}$ which is independent of $\mu_{\St}$. The necessary condition for $z^\star_{\Itb} = 1$ is $\Delta U[\Itb](1,1;\mu_{\St}) \leq 0$, or equivalently, $g(1,\mu_{\St})\leq 0$, which yields
%\begin{align*}
%    & (1-\pi^+[\St | \Itb])(C_{\Ut} - C_{\Pt}) + \pi^+[\St | \Itb] \Delta U [\Stb] \leq 0.
%\end{align*}
%Thus, we must necessarily have $\Delta U [\Stb] \leq 0$ which implies $z^\star_{\Stb} = 1$. Substituting $\pi^+[\St | \Itb]$ from \eqref{eq:pi_plus_s_ibar} in the above inequality yields
\begin{align*}
    & y^\star(1,1) (C_{\Ut} - C_{\Pt}) \leq 
    \\ & \qquad (1-\mu_{\St})(1-y^\star(1,1)) (-\Delta U[\Stb](1,1;\mu_{\St}))
    \\ \iff & 1-\mu_{\St} \geq \frac{y^\star(1,1) (C_{\Ut} - C_{\Pt})}{(1-y^\star(1,1)) (-\Delta U[\Stb](1,1;\mu_{\St}))}
    \\ & \qquad = \frac{y^\star(1,1) (C_{\Ut} - C_{\Pt})}{(1-y^\star(1,1)) (C_{\Pt} - (1-\alpha) L \beta_{\Ut} y^\star(1,1))}
    \\ & \qquad = \frac{(\betau - \gamma) (C_{\Ut} - C_{\Pt})}{\gamma (C_{\Pt} - (1-\alpha) L (\beta_{\Ut} -\gamma))}
    \\ \iff & \mu_{\St} < \mu^{\min}_{\St}. 
\end{align*}
In addition, we must have $\mu^{\min}_{\St}>0$; otherwise, the above condition is not satisfied for any feasible value of $\mu_{\St}$.

Furthermore, we require the R.H.S. of the above inequality to be at most $1$ to ensure that $\mu_{\St} >0$. In addition, the condition $\Delta U [\Stb] \leq 0$ yields
\begin{align*}
    & (1-\alpha) L \beta_{\Ut} y^\star(1,1)- C_{\Pt} \leq 0
    \\ \implies & 1 - \frac{\gamma}{\betau} \leq \frac{C_{\Pt}}{L(1-\alpha)\betau}.
\end{align*}

For sufficiency, suppose the hypothesis stated in the proposition simultaneously hold true. Let $(y^\star(z^\star_{\Stb},z^\star_{\Itb}), z^\star_{\Stb},z^\star_{\Itb})$ be a SNE. We compute 
\begin{align*}
\Delta U[\Stb] & = (1-\alpha) L (\beta_{\Pt} + (\beta_{\Ut} - \beta_{\Pt}) z^\star_{\Itb}) y^\star(z^\star_{\Stb},z^\star_{\Itb})- C_{\Pt}
\\ & \leq (1-\alpha) L (\beta_{\Ut}) y^\star(1,1)- C_{\Pt} < 0,
\end{align*}
which follows from the monotonicity of $y^\star(z^\star_{\Stb},z^\star_{\Itb})$ in both of its arguments. Consequently, we must have $z^\star_{\Stb} = 1$. Note further that
\begin{align*}
1-\mu_{\St} & \geq \frac{(\betau - \gamma) (C_{\Ut} - C_{\Pt})}{\gamma (C_{\Pt} - (1-\alpha) L (\beta_{\Ut} -\gamma))}
\\ & = \frac{y^\star(1,1) (C_{\Ut} - C_{\Pt})}{(1-y^\star(1,1)) (C_{\Pt} - (1-\alpha) L \beta_{\Ut} y^\star(1,1))}
\\ & \geq \frac{y^\star(z^\star_{\Stb},z^\star_{\Itb}) (C_{\Ut} - C_{\Pt})}{(1-y^\star(z^\star_{\Stb},z^\star_{\Itb})) (C_{\Pt} - (1-\alpha) L \beta_{\Ut} y^\star(z^\star_{\Stb},z^\star_{\Itb}))},
\end{align*}
as the numerator is strictly increasing in $y^\star$ and the denominator is positive and strictly decreasing in $y^\star$. It follows from earlier discussion that the above inequality is equivalent to
\begin{align*}
    & (1-\pi^+[\St | \Itb])(C_{\Ut} - C_{\Pt}) + \pi^+[\St | \Itb] \Delta U [\Stb] \leq 0.
\end{align*}
at $(y^\star(z^\star_{\Stb},z^\star_{\Itb}), z^\star_{\Stb},z^\star_{\Itb})$ which implies $z^\star_{\Itb}=1$.
\end{proof}

We now examine equilibria with $\zsbar=1$. In this regime, it is possible for $\zibar$ to be larger than $0$. In addition, $\mu_{\St}$ also plays a significant role in the equilibrium analysis. We define the following quantities of interest with a slight abuse of notation to highlight the dependence on $\mu_{\St}$.
\begin{align*}
    & \beta_{\mathtt{eff}}(1,z_{\Itb};\mu_{\St}) = (\betap + (\betau - \betap)z_{\Itb}) \nonumber
    \\ & \qquad \qquad \qquad \times (\alpha+(1-\alpha)(\mu_{\St} + z_{\Itb}(1-\mu_{\St}))),
    \\ & y^\star(1,z_{\Itb};\mu_{\St}) = 1-\frac{\gamma}{\beta_{\mathtt{eff}}(1,z_{\Itb};\mu_{\St})},
    \\ & \pi^{+}[\St|\Itb](1,z_{\Itb};\mu_{\St}) = 1 - \frac{y^\star(1,z_{\Itb};\mu_{\St})}{1-\mu_{\St}+\mu_{\St}y^\star(1,z_{\Itb};\mu_{\St})},
    \\ & \Delta U[\Stb](1,z_{\Itb};\mu_{\St}) = (1-\alpha) L (\beta_{\Pt} + (\beta_{\Ut} - \beta_{\Pt}) z_{\Itb}) \nonumber
    \\ & \qquad \qquad \qquad \qquad \quad \times y^\star(1,z_{\Itb};\mu_{\St}) - C_{\Pt},
    \\ & \Delta U[\Itb](1,z_{\Itb};\mu_{\St}) = (1-\pi^+[\St | \Itb](1,z_{\Itb};\mu_{\St}))(C_{\Ut} - C_{\Pt}) \nonumber
    \\ & \qquad \qquad \qquad + \pi^+[\St | \Itb](1,z_{\Itb};\mu_{\St}) \Delta U [\Stb](1,z_{\Itb};\mu_{\St})
    \\ \Rightarrow & (1-\mu_{\St}+\mu_{\St}y^\star(1,z_{\Itb};\mu_{\St})) \Delta U[\Itb](1,z_{\Itb};\mu_{\St}) = g(z_{\Itb};\mu_{\St}),
\end{align*}
where 
\begin{align}
& g(z_{\Itb};\mu_{\St}) := y^\star(1,z_{\Itb};\mu_{\St}) (C_{\Ut} - C_{\Pt}) \nonumber
\\ & \quad - (1-\mu_{\St})(1-y^\star(1,z_{\Itb};\mu_{\St}))(-\Delta U [\Stb](1,z_{\Itb};\mu_{\St})). \label{eq:function_g_zi_mus}
\end{align}

From the above expressions, it is easy to see that $\beta_{\mathtt{eff}}(1,z_{\Itb};\mu_{\St})$ is monotonically increasing in both $z_{\Itb}$ and $\mu_{\St}$. Consequently, $y^\star(1,z_{\Itb};\mu_{\St})$ and $\Delta U[\Stb](1,z_{\Itb};\mu_{\St})$ are monotonically increasing in both $z_{\Itb}$ and $\mu_{\St}$. Similarly, $\pi^{+}[\St|\Itb](1,z_{\Itb};\mu_{\St})$ is decreasing in $y^\star(1,z_{\Itb};\mu_{\St})$. Finally, when $\Delta U[\Stb](1,z_{\Itb};\mu_{\St}) < 0$, $g(z_{\Itb};\mu_{\St})$ is monotonically increasing in both $z_{\Itb}$ and $\mu_{\St}$, and $g(z_{\Itb};1) > 0$. In addition, the sign of $\Delta U[\Itb](1,z_{\Itb};\mu_{\St})$ is determined by the sign of $g(z_{\Itb};\mu_{\St})$. We now define
\begin{align}\label{eq:def_mus_max}
    \mu^{\max}_{\St} := \begin{cases}
        & 0, \qquad \text{if} \quad g(0,0) \geq 0
        \\ & \mu^{\star}_{\St}, \quad \text{where} \quad g(0,\mu^{\star}_{\St}) = 0, \mu^{\star}_{\St} \in (0,1). 
    \end{cases}
\end{align}
In particular, $\mu^{\max}_{\St} = 0$ when $g(0,\mu_{\St}) \geq g(0,0) \geq 0$ for all $\mu_{\St} \in [0,1]$. Otherwise, if $g(0,0) < 0$ and $g(0,1)>0$, there exists a unique $\mu^{\star}_{\St} \in (0,1)$ for which $g(0,\mu^{\star}_{\St}) = 0$. In this case, we define $\mu^{\max}_{\St} = \mu^{\star}_{\St}$.

We leverage the above properties to characterize equilibrium with $\zibar=0$ and $\zsbar=1$ in the following result. 

\begin{proposition}
    $(y^\star(1,0),1,0)$ is a SNE if and only if 
    \begin{align*}
        &  \mu_{\St} \in [\mu^{\max}_{\St},1], \quad \text{and} \quad 1 - \frac{\gamma}{\betap (\alpha + (1 - \alpha) \mu_{\St})} \leq \yint. 
    \end{align*} 
    \label{prop:zi_zero_zs_one}
\end{proposition}

\begin{proof}
   Necessary condition for $\zsbar=1$ is
    \begin{align*}
        & \Delta U[\Stb](1,0;\mu_{\St}) \leq 0
        \\ \iff & (1-\alpha) L \betap y^\star(1,0) \leq C_{\Pt}
        \\ \iff & y^\star(1,0) = 1-\frac{\gamma}{\betap(\alpha+(1-\alpha)\mu_{\St})} \leq \yint. 
    \end{align*} 
    Similarly, necessary condition for $\zibar=0$ is
    \begin{align*}
        \Delta U[\Itb](1,0;\mu_{\St}) \geq 0 & \iff g(0,\mu_{\St}) \geq 0 
        \\ & \iff \mu_{\St} \in [\mu^{\max}_{\St},1]. 
    \end{align*}
    The last implication follows from the definition of $\mu^{\max}_{\St}$ in \eqref{eq:def_mus_max} and monotonicity of $g(z_{\Itb},\mu_{\St})$ defined in \eqref{eq:function_g_zi_mus} in $\mu_{\St}$. 
 
    The necessary conditions are also sufficient in this case. Since $g(z_{\Itb},\mu_{\St})$ is monotonically increasing in $z_{\Itb}$, 
    $$\Delta U[\Itb](1,0;\mu_{\St}) \geq 0 \implies \Delta U[\Itb](1,z_{\Itb};\mu_{\St}) > 0$$ for every $z_{\Itb} \in (0,1]$. As a result, any $z_{\Itb} \neq 0$ cannot be present at a SNE. When $z_{\Itb}=0$, we have 
    $$\Delta U[\Stb](z_{\Stb},0;\mu_{\St}) < \Delta U[\Stb](1,0;\mu_{\St}) \leq 0$$ 
    for any $z_{\Stb} \in [0,1)$; the second inequality above follows from our hypothesis on $\yint$. As a result, $z_{\Stb} \neq 1$ cannot be present at a SNE. This concludes the proof.
\end{proof}

\begin{proposition}\label{prop:zibar_interior}
    $(y^\star(1,\zidag),1,\zidag)$ with $\zidag \in (0,1)$ being the unique solution satisfying $g(\zidag,\mu_{\St})=0$ is a SNE if and only if 
    \begin{equation*}
        \mu^{\max}_{\St} > 0 \quad \text{and} \quad \mu_{\St} \in (\mu^{\min}_{\St},\mu^{\max}_{\St}) \cap [0,1].
    \end{equation*} 
\end{proposition}

\vspace{0.2cm}

\begin{proof}
    We first show the sufficiency part. Recall that when $\mu^{\max}_{\St} > 0$, then $g(0,\mu^{\max}_{\St})=0$. From the monotonicity of $g$, it follows that $g(0,\mu_{\St}) < 0$ for all $\mu_{\St} < \mu^{\max}_{\St}$. Therefore, $\zibar=0$ can not arise at the SNE. Similarly, when $\mu_{\St} > \mu^{\min}_{\St}$, $g(1,\mu_{\St}) > 0$ which implies that $\zibar=1$ can not arise at the SNE. 

    Nevertheless, since $g(z_{\Itb},\mu_{\St})$ is monotonically increasing in $z_{\Itb}$, there exists a unique $\zidag \in (0,1)$ at which $g(\zidag,\mu_{\St})=0$, or equivalently, $\Delta U[\It](1,\zidag;\mu_{\St}) = 0$. This further implies that $\Delta U[\St](1,\zidag;\mu_{\St}) < 0$ or $\zsbar=1$. 

    We next show the necessity. Since $\zidag \in (0,1)$, we must have $\Delta U[\It](1,\zidag;\mu_{\St}) = 0$ or equivalently, $g(\zidag,\mu_{\St})=0$. Due to monotonicity of $g$ in the first argument, the above condition implies
    \begin{align*}
       & g(0,\mu_{\St})<0 \quad \text{and} \quad g(1,\mu_{\St})>0 
       \\ & \iff \mu_{\St} \in (\mu^{\min}_{\St},\mu^{\max}_{\St}). 
    \end{align*}
    Finally, $\Delta U[\St](1,\zidag;\mu_{\St}) < 0$ implies 
    \begin{align*} 
    & (1-\alpha) L (\beta_{\Pt} + (\beta_{\Ut} - \beta_{\Pt}) \zidag) y^\star(1,\zidag;\mu_{\St}) - C_{\Pt} < 0
    \\ \implies & C_{\Pt} > (1-\alpha) L \beta_{\Pt} y^\star(1,0;\mu_{\St})
    \\ \iff & \yint > 1-\frac{\gamma}{\betap (\alpha + (1 - \alpha) \mu_{S})},
    \end{align*}
    which does not contradict the regime in an earlier Proposition. 
\end{proof}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We now examine the equilibrium where all agents adopt protection. 

\begin{proposition}
    $(y^*_{\Pt},0,0)$ is a SNE if and only if $y^*_{\Pt} > \yint$. 
    \label{prop:y^*_p}
\end{proposition}
\begin{proof}
First observe that $y^\star(0,0) = y^*_{\Pt}$. Note that the necessary condition for $z^\star_{\Stb} = 0$ is $\Delta U[\Stb] \geq 0$, or equivalently, 
\begin{align*}
    & (1-\alpha) L (\beta_{\Pt} + (\beta_{\Ut} - \beta_{\Pt}) z^\star_{\Itb}) y^*_{\Pt}- C_{\Pt} \geq 0
    \\ \iff & (1-\alpha) L (\beta_{\Pt}) y^*_{\Pt}- C_{\Pt} \geq 0
    \\ \iff & y^*_{\Pt} \geq \frac{C_{\Pt}}{(1-\alpha) L (\beta_{\Pt})} = \yint. 
\end{align*}
For sufficiency, assume that $y^*_{\Pt} > \yint$. Let $z^\star_{\Stb}$ and $z^\star_{\Itb}$ be the proportions of nodes who remain unprotected upon receiving signal $\Stb$ and $\Itb$, respectively. Then, $y^\star(z^\star_{\Stb},z^\star_{\Itb}) \geq y^\star(0,0) = y^*_{\Pt}$ since $y^\star(z_{\Stb},z_{\Itb})$ is monotonically increasing in $\beta_{\mathtt{eff}}(z_{\Stb},z_{\Itb})$, and the latter is monotonically increasing in both $z_{\Stb}$ and $z_{\Itb}$. We now compute 
\begin{align*}
\Delta U[\Stb] & = (1-\alpha) L (\beta_{\Pt} + (\beta_{\Ut} - \beta_{\Pt}) z^\star_{\Itb}) y^\star(z^\star_{\Stb},z^\star_{\Itb})- C_{\Pt}
\\ & \geq (1-\alpha) L (\beta_{\Pt}) y^\star(0,0)- C_{\Pt} > 0,
\end{align*}
under our hypothesis. Now, it follows from Proposition \ref{prop:unstable} that $z^\star_{\Itb} = 0$. This concludes the proof.
\end{proof}

\begin{proposition}
    $(\yint, \zsdag, 0)$ is a SNE if and only if 
    \begin{align*}
        & 1 - \frac{\gamma}{\alpha \betap} < \yint < 1 - \frac{\gamma}{\betap (\alpha + (1 - \alpha) \mu_{S})},% < 1 - \frac{\gamma}{\betap},
    \end{align*} 
    where $\zsdag = \frac{\gamma - \alpha \betap (1 - \yint)}{\betap (1 - \alpha) (1 - \yint) \mu_{S}} \in (0, 1)$.
    \label{prop:y*_int}
\end{proposition}
\begin{proof}
When $\zsdag \in (0,1)$, it follows from Proposition \ref{prop:unstable} that $\zibar = 0$. The necessary condition pertaining to $\zsdag \in (0, 1)$ is $\Delta U[\Stb] = 0$, or equivalently,
\begin{align*}
    & (1-\alpha) L (\beta_{\Pt} + (\beta_{\Ut} - \beta_{\Pt}) z_{\Itb}) y^\star(\zsdag,0)- C_{\Pt} = 0
    \\ \iff & (1-\alpha) L \beta_{\Pt} y^\star(\zsdag,0)- C_{\Pt} = 0
    \\ \iff & y^\star(\zsdag,0) = \frac{C_{\Pt}}{(1-\alpha) L \beta_{\Pt}} = \yint
    \\ \iff & 1-\frac{\gamma}{\betap (\alpha+(1-\alpha)(\zsdag \mu_{\St}))} = \yint 
    \\ \iff & \zsdag = \frac{\gamma - \alpha \betap (1 - \yint)}{\betap (1 - \alpha) (1 - \yint) \mu_{S}}. 
\end{align*}
Since $y^\star(\zsbar,\zibar)$ is monotonically increasing in both of its arguments, we must have
\begin{align*}
    & y^\star(0,0) < y^\star(\zsdag,0) < y^\star(1,0)
    \\ \implies & 1-\frac{\gamma}{\alpha \betap} < \yint < 1-\frac{\gamma}{ \betap (\alpha+(1-\alpha)\mu_{\St})}. 
\end{align*}
In other words, when $\yint$ lies in the above range, there exists a unique $\zsdag \in (0,1)$ satisfying $y^\star(\zsdag,0) = \yint$. 

For sufficiency, suppose the hypothesis stated in the proposition hold true. It follows from \eqref{eq:del_Sbar} that the function
$$
\Delta U[\Stb](z_{\Stb},z_{\Itb}) := (1-\alpha) L (\beta_{\Pt} + (\beta_{\Ut} - \beta_{\Pt}) z_{\Itb}) y^\star(z_{\Stb},z_{\Itb})- C_{\Pt}
$$
is monotonically increasing in both of its arguments. Under our hypothesis, we have
\begin{align*}
& \Delta U[\Stb](0,0) < 0 \implies \zsbar \neq 0, 
\\ & \Delta U[\Stb](1,z_{\Itb}) \geq \Delta U[\Stb](1,0) > 0 \implies \zsbar \neq 1.
\end{align*}
However, due to the monotonicity of $\Delta U[\Stb](z_{\Stb},0)$, there exists a unique $\zsbar \in (0,1)$ at which $\Delta U[\Stb](\zsbar,0) = 0$, which yields $y^\star(\zsbar,0) = \yint$ and $\zsbar = \zsdag$. This concludes our proof.
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We now analyse the equilibrium points based on the utilities and the conditions under which they exist.

\begin{itemize}

\item \textbf{Case: 2}\vspace{5pt}
    \\\fbox{\begin{minipage}{\linewidth}
    $z^*_{\bar{\texttt{S}}} = 1$,  $z^*_{\bar{\texttt{I}}} = 1$, $y^* = 1 - \frac{\gamma}{\beta_{\texttt{U}}}$ is stable when $(1 - \alpha) L \beta_{\texttt{U}} y^* < C_{\texttt{P}}$, $\mu_{S} < 1 - \frac{(\beta_{\texttt{U}} - \gamma) (C_{\texttt{P}} -  C_{\texttt{U}})}{\gamma ((1 - \alpha) L (\beta_{\texttt{U}} - \gamma) - C_{\texttt{P}})}$ and $\frac{(\beta_{\texttt{U}} - \gamma) (C_{\texttt{P}} -  C_{\texttt{U}})}{\gamma ((1 - \alpha) L (\beta_{\texttt{U}} - \gamma) - C_{\texttt{P}})} < 1$, must simultaneously hold. 
    \end{minipage}}\vspace{5pt}
    \\This equilibrium point reflects the condition when none of the agents adopt protection. This is possible when both $U[\bar{\texttt{S}}, \texttt{P}] < U[\bar{\texttt{S}}, \texttt{U}] $ and $U[\bar{\texttt{I}}, \texttt{P}] < U[\bar{\texttt{I}}, \texttt{U}] $ are satisfied. From \eqref{eq:zs} and \eqref{eq:zi} we obtain $z^*_ {\texttt{S}} = z^*_ {\texttt{I}} = 1$. In this case $y^* = 1 - \frac{\gamma}{\beta_{\texttt{U}}}$ is the infection state equilibrium, and $\texttt{F}[\texttt{S}, \texttt{U}] = -L \beta_{\texttt{U}} y^*$. We proceed the similar way as in previous case to obtain the conditions.
    \begin{align}
        &(1 - \alpha) L \beta_{\texttt{U}} y^* < C_{\texttt{P}},
        \label{eq:del_Sbar_cost2}
       \\ &(1 - \mu_{S}) (1 - y^*) ((1 - \alpha) L \beta_{\texttt{U}} y^* - C_{\texttt{P}}) < y^* ( C_{\texttt{P}} -  C_{\texttt{U}})\nonumber\\&\implies \mu_{S} < 1 - \frac{y^* (C_{\texttt{P}} -  C_{\texttt{U}})}{(1 - y^*) ((1 - \alpha) L \beta_{\texttt{U}} y^* - C_{\texttt{P}})}. 
        \label{eq:del_Ibar_cost2}
    \end{align}
    From Assumption \ref{assump:cost} and \eqref{eq:del_Sbar_cost2} it is clear that $\frac{y^* (C_{\texttt{P}} -  C_{\texttt{U}})}{(1 - y^*) ((1 - \alpha) L \beta_{\texttt{U}} y^* - C_{\texttt{P}})}$ is positive, which results in $\mu_{S} < 1 - \frac{(\beta_{\texttt{U}} - \gamma) (C_{\texttt{P}} -  C_{\texttt{U}})}{\gamma ((1 - \alpha) L (\beta_{\texttt{U}} - \gamma) - C_{\texttt{P}})}$. For the equilibrium point to exist such that $\mu_{S} \in (0, 1)$, it is mandatory that $\frac{(\beta_{\texttt{U}} - \gamma) (C_{\texttt{P}} -  C_{\texttt{U}})}{\gamma ((1 - \alpha) L (\beta_{\texttt{U}} - \gamma) - C_{\texttt{P}})} < 1$ also holds.

    

    
    

\item \textbf{Case: 4}\vspace{5pt}
    \\\fbox{\begin{minipage}{\linewidth}
    $z^*_{\bar{\texttt{S}}} = 1$,  $z^*_{\bar{\texttt{I}}} = 0$, $y^* = 1 - \frac{\gamma}{\beta_{\texttt{P}} (\mu_S + (1 - \mu_S) \alpha)}$ is stable when either set of conditions holds:
    \begin{itemize}
        \item [$\blacksquare$] $(1 - \alpha) L \beta_{\texttt{P}} - C_{\texttt{P}} > 0$, $\mu_{S} < \frac{\gamma (1 - \alpha) L - \alpha (1 - \alpha) L \beta_{\texttt{P}} + \alpha C_{\texttt{P}}}{(1 - \alpha) ((1 - \alpha) L \beta_{\texttt{P}} - C_{\texttt{P}})}$ and $0 < \frac{\gamma (1 - \alpha) L - \alpha (1 - \alpha) L \beta_{\texttt{P}} + \alpha C_{\texttt{P}}}{(1 - \alpha) ((1 - \alpha) L \beta_{\texttt{P}} - C_{\texttt{P}})} \leq 1$ simultaneously hold, or,
        \item [$\blacksquare$] $(1 - \alpha) L \beta_{\texttt{P}} - C_{\texttt{P}} < 0$, $\mu_{S} > \frac{\gamma (1 - \alpha) L - \alpha (1 - \alpha) L \beta_{\texttt{P}} + \alpha C_{\texttt{P}}}{(1 - \alpha) ((1 - \alpha) L \beta_{\texttt{P}} - C_{\texttt{P}})}$ and $0 \leq \frac{\gamma (1 - \alpha) L - \alpha (1 - \alpha) L \beta_{\texttt{P}} + \alpha C_{\texttt{P}}}{(1 - \alpha) ((1 - \alpha) L \beta_{\texttt{P}} - C_{\texttt{P}})} < 1$ simultaneously hold.
    \end{itemize}
    
     
    \end{minipage}}\vspace{5pt}




    $z^*_{\bar{\texttt{S}}} = 1$ and  $z^*_{\bar{\texttt{I}}} = 0$  
     \\This equilibrium point gives the condition when all agents receiving signal of being infected adopt protection, whereas, those receiving signal of being susceptible remain unprotected. This is possible when both $U[\bar{\texttt{S}}, \texttt{P}] < U[\bar{\texttt{S}}, \texttt{U}] $ and $U[\bar{\texttt{I}}, \texttt{P}] > U[\bar{\texttt{I}}, \texttt{U}] $ are satisfied. $z^*_{\bar{\texttt{S}}} = 1, z^*_{\bar{\texttt{I}}} = 0$ yields $z^*_{{\texttt{S}}} = \mu_S, z^*_{{\texttt{I}}} = 0$, and the equilibrium point obtained is $y^* = 1 - \frac{\gamma}{\beta_{\texttt{P}} (\mu_S + (1 - \mu_S) \alpha)}$. Also, under these conditions we obtain $\texttt{F}[\texttt{S}, \texttt{U}] = -L \beta_{\texttt{P}} y^*$.

     \begin{align}
        &(1 - \alpha) L \beta_{\texttt{P}} y^* < C_{\texttt{P}},
        \label{eq:del_Sbar_cost4}
       \\ &(1 - \mu_{S}) (1 - y^*) ((1 - \alpha) L \beta_{\texttt{P}} y^* - C_{\texttt{P}}) > y^* ( C_{\texttt{P}} -  C_{\texttt{U}})\nonumber\\&\implies \mu_{S} > 1 - \frac{y^* (C_{\texttt{P}} -  C_{\texttt{U}})}{(1 - y^*) ((1 - \alpha) L \beta_{\texttt{P}} y^* - C_{\texttt{P}})}. 
        \label{eq:del_Ibar_cost4}
    \end{align}
    From Assumption \ref{assump:cost} and \eqref{eq:del_Sbar_cost4} we get $\frac{y^* (C_{\texttt{P}} -  C_{\texttt{U}})}{(1 - y^*) ((1 - \alpha) L \beta_{\texttt{P}} y^* - C_{\texttt{P}})}$ as positive. Substituting $y^* = 1 - \frac{\gamma}{\beta_{\texttt{P}} (\mu_S + (1 - \mu_S) \alpha)}$ in \eqref{eq:del_Sbar_cost4} results in 
    \begin{align}
        &\frac{\gamma (1 - \alpha) L}{\alpha + (1 - \alpha) \mu_{S}} > (1 - \alpha) L \beta_{\texttt{P}} - C_{\texttt{P}}, \nonumber
        \\&\implies \mu_{S} < \frac{\gamma (1 - \alpha) L - \alpha (1 - \alpha) L \beta_{\texttt{P}} + \alpha C_{\texttt{P}}}{(1 - \alpha) ((1 - \alpha) L \beta_{\texttt{P}} - C_{\texttt{P}})}, \;\; \nonumber
        \\&\textrm{when}\; (1 - \alpha) L \beta_{\texttt{P}} - C_{\texttt{P}} > 0; \;\textrm{or}, 
        \label{eq:case4_th1}
        \\&\mu_{S} > \frac{\gamma (1 - \alpha) L - \alpha (1 - \alpha) L \beta_{\texttt{P}} + \alpha C_{\texttt{P}}}{(1 - \alpha) ((1 - \alpha) L \beta_{\texttt{P}} - C_{\texttt{P}})}, \;\; \nonumber
        \\&\textrm{when}\; (1 - \alpha) L \beta_{\texttt{P}} - C_{\texttt{P}} < 0.
        \label{eq:case4_th2}
    \end{align}
    Also, the above equilibrium point will be stable when the threshold of $\mu_{S}$ defined by \eqref{eq:case4_th1}, or \eqref{eq:case4_th2} eventually leads to $\mu_{S} \in [0, 1]$. Thus, when $(1 - \alpha) L \beta_{\texttt{P}} - C_{\texttt{P}} > 0$ holds, we must have $0 < \frac{\gamma (1 - \alpha) L - \alpha (1 - \alpha) L \beta_{\texttt{P}} + \alpha C_{\texttt{P}}}{(1 - \alpha) ((1 - \alpha) L \beta_{\texttt{P}} - C_{\texttt{P}})} \leq 1$. Similarly, when $(1 - \alpha) L \beta_{\texttt{P}} - C_{\texttt{P}}$ is true, $0 \leq \frac{\gamma (1 - \alpha) L - \alpha (1 - \alpha) L \beta_{\texttt{P}} + \alpha C_{\texttt{P}}}{(1 - \alpha) ((1 - \alpha) L \beta_{\texttt{P}} - C_{\texttt{P}})} < 1$ must be satisfied to guarantee stability of the equilibrium point.
    
    
    
    
    
    
    %Thus, we solve equation \eqref{eq:del_Ibar_cost4} and $y^* = 1 - \frac{\gamma}{\beta_{\texttt{P}} (\mu_S + (1 - \mu_S) \alpha)}$ to determine the range of $\mu_{S}$.


    


   



     \item \textbf{Case: 8}\vspace{5pt}
    \\\fbox{\begin{minipage}{\linewidth}
    $z^*_{\bar{\texttt{S}}} = z^\dagger_{\bar{\texttt{S}}}$,  $z^*_{\bar{\texttt{I}}} = 0$, $y^* = 1 - \frac{\gamma}{ \beta_{\texttt{P}} (\alpha + (1 - \alpha) \mu_{S} z^\dagger_{\bar{\texttt{S}}})}$ is stable. \um{But I can't characterize it till now} 
    \end{minipage}}\vspace{5pt}
    \\This is possible when both $U[\bar{\texttt{S}}, \texttt{P}] = U[\bar{\texttt{S}}, \texttt{U}] $ and $U[\bar{\texttt{I}}, \texttt{P}] > U[\bar{\texttt{I}}, \texttt{U}] $ are satisfied. From \eqref{eq:zs} and \eqref{eq:zi} we obtain $z^*_ {\texttt{S}} = z^\dagger_{\bar{\texttt{S}}} \mu_{S} , z^*_ {\texttt{I}} = 0$. The infection state equilibrium point obtained is $y^* = 1 - \frac{\gamma}{ \beta_{\texttt{P}} (\alpha + (1 - \alpha) \mu_{S} z^\dagger_{\bar{\texttt{S}}})}$, whereas, $\texttt{F}[\texttt{S}, \texttt{U}] = -L \beta_{\texttt{P}} y^*$.
    
     \begin{align}
        &(1 - \alpha) L \beta_{\texttt{P}} y^* = C_{\texttt{P}},
        \label{eq:del_Sbar_cost8}
       \\ &(1 - \mu_{S}) (1 - y^*) ((1 - \alpha) L \beta_{\texttt{P}} y^* - C_{\texttt{P}}) > y^* ( C_{\texttt{P}} -  C_{\texttt{U}}) \nonumber
       \\&\implies 0 > y^* (C_{\texttt{P}} -  C_{\texttt{U}}). 
        \label{eq:del_Ibar_cost8}
    \end{align}
    Equation \eqref{eq:del_Sbar_cost8} is always satisfied by Assumption \ref{assump:cost}, irrespective of any $\mu_{S} \in [0, 1]$. Thus, the equilibrium point is stable with $y^* = \frac{C_{\texttt{P}}}{(1 - \alpha) L \beta_{\texttt{P}}}$. Also, $y^* = 1 - \frac{\gamma}{ \beta_{\texttt{P}} (\alpha + (1 - \alpha) \mu_{S} z^\dagger_{\bar{\texttt{S}}})}$ yields $z^\dagger_{\bar{\texttt{S}}} = \frac{\gamma - \alpha (1 - y^*)}{\mu_{S} (1 - \alpha) (1 - y^*)}$.


    \item \textbf{Case: 9}\vspace{5pt}
    \\\fbox{\begin{minipage}{\linewidth}
    $z^*_{\bar{\texttt{S}}} = 1$,  $z^*_{\bar{\texttt{I}}} = z^\dagger_{\bar{\texttt{I}}}$, $y^* = 1 - \frac{\gamma}{ (\beta_{\texttt{P}} + (\beta_{\texttt{U}} - \beta_{\texttt{P}}) z^\dagger_{\bar{\texttt{I}}}) (\alpha + (1 - \alpha) (\mu_{S} + z^\dagger_{\bar{\texttt{I}}} (1 - \mu_{S})))}$. 
    \end{minipage}}\vspace{5pt}
    \\This is possible when both $U[\bar{\texttt{S}}, \texttt{P}] < U[\bar{\texttt{S}}, \texttt{U}] $ and $U[\bar{\texttt{I}}, \texttt{P}] = U[\bar{\texttt{I}}, \texttt{U}] $ are satisfied. From \eqref{eq:zs} and \eqref{eq:zi} we obtain $z^*_ {\texttt{S}} = \mu_{S} + z^\dagger_{\bar{\texttt{I}}} (1 - \mu_{S}) , z^*_ {\texttt{I}} = z^\dagger_{\bar{\texttt{I}}}$. The infection state equilibrium point obtained is $y^* = 1 - \frac{\gamma}{ (\beta_{\texttt{P}} + (\beta_{\texttt{U}} - \beta_{\texttt{P}}) z^\dagger_{\bar{\texttt{I}}}) (\alpha + (1 - \alpha) (\mu_{S} + z^\dagger_{\bar{\texttt{I}}} (1 - \mu_{S})))}$, whereas, $\texttt{F}[\texttt{S}, \texttt{U}] = -L (\beta_{\texttt{P}} + (\beta_{\texttt{U}} - \beta_{\texttt{P}}) z^\dagger_{\bar{\texttt{I}}}) y^*$.
    
     \begin{align}
        &(1 - \alpha) L (\beta_{\texttt{P}} + (\beta_{\texttt{U}} - \beta_{\texttt{P}}) z^\dagger_{\bar{\texttt{I}}}) y^* < C_{\texttt{P}},
        \label{eq:del_Sbar_cost9}
       \\ &(1 - \mu_{S}) (1 - y^*) ((1 - \alpha) L (\beta_{\texttt{P}} + (\beta_{\texttt{U}} - \beta_{\texttt{P}}) z^\dagger_{\bar{\texttt{I}}}) y^* - C_{\texttt{P}}) \nonumber
       \\&= y^* ( C_{\texttt{P}} -  C_{\texttt{U}}) \nonumber
       \\&\implies \mu_{S} = 1 - \frac{y^* (C_{\texttt{U}} -  C_{\texttt{P}})}{(1 - y^*) (C_{\texttt{P}} - (1 - \alpha) L (\beta_{\texttt{P}} + (\beta_{\texttt{U}} - \beta_{\texttt{P}}) z^\dagger_{\bar{\texttt{I}}}) y^*)}. 
        \label{eq:del_Ibar_cost9}
    \end{align}
   
    
    
    

    
%     \begin{align*}
%         U[\bar{\texttt{I}}, \texttt{P}] &= \alpha w \texttt{F}[\texttt{S}, \texttt{U}] - C_\texttt{P},   \;\;\;\; U[\bar{\texttt{I}}, \texttt{U}] = w \texttt{F}[\texttt{S}, \texttt{U}] - (1 - w) C_\texttt{U}, \;\;\;\; \texttt{F}[\texttt{S}, \texttt{U}] = -L \beta_{\texttt{P}} y.
%     \end{align*}
%     The difference in utilities leads to
%     \begin{align}
%         &U[\bar{\texttt{I}}, \texttt{P}] - U[\bar{\texttt{I}}, \texttt{U}] > 0, \nonumber
%         \\&\implies w < \frac{C_\texttt{P} - C_\texttt{U}}{(1 - \alpha) L \beta_{\texttt{P}} y - C_\texttt{U}},
%         \label{eq:del_u_i3}
%        \\&U[\bar{\texttt{S}}, \texttt{P}] - U[\bar{\texttt{S}}, \texttt{U}] < 0, \nonumber
%         \\&\implies v < \frac{C_\texttt{P}}{(1 - \alpha) L \beta_{\texttt{P}} y}.
%         \label{eq:del_u_s3}
%     \end{align}
 
% We have $w = \frac{(1 - \mu_S)(1 - y^*)}{(1 - \mu_S)(1 - y^*) + y^*}$ and $v = 1$. We define $A_{\texttt{U,P}} = \frac{C_\texttt{P} - C_\texttt{U}}{(1 - \alpha) L \beta_{\texttt{P}} y^* - C_\texttt{U}}$. Also, $0 < A_{\texttt{U,P}} < 1$ holds. Thus, \eqref{eq:del_u_i3} is rewritten as $\frac{(1 - \mu_S)(1 - y^*)}{(1 - \mu_S)(1 - y^*) + y^*} < A_{\texttt{U,P}}$, which on simplification yields $\mu_S < 1 - \frac{A_{\texttt{U,P}} y^*}{(1 - y^*) (1 - A_{\texttt{U,P}})}$, or, $\mu_S < 1 - \frac{(C_\texttt{P} - C_\texttt{U}) (\beta_{\texttt{P}} (\mu_s + (1 - \mu_S) \alpha) - \gamma) (\mu_s + (1 - \mu_S) \alpha)}{\gamma ((1 - \alpha) L  (\beta_{\texttt{P}} (\mu_s + (1 - \mu_S) \alpha) - \gamma) - (\mu_s + (1 - \mu_S) \alpha) C_{\texttt{P}})}$. Thus, the above equilibrium point is obtained if and only if both $\mu_S < 1 - \frac{(C_\texttt{P} - C_\texttt{U}) (\beta_{\texttt{P}} (\mu_s + (1 - \mu_S) \alpha) - \gamma) (\mu_s + (1 - \mu_S) \alpha)}{\gamma ((1 - \alpha) L  (\beta_{\texttt{P}} (\mu_s + (1 - \mu_S) \alpha) - \gamma) - (\mu_s + (1 - \mu_S) \alpha) C_{\texttt{P}})}$ and $1 - \frac{(C_\texttt{P} - C_\texttt{U}) (\beta_{\texttt{P}} (\mu_s + (1 - \mu_S) \alpha) - \gamma) (\mu_s + (1 - \mu_S) \alpha)}{\gamma ((1 - \alpha) L  (\beta_{\texttt{P}} (\mu_s + (1 - \mu_S) \alpha) - \gamma) - (\mu_s + (1 - \mu_S) \alpha) C_{\texttt{P}})} > 0$ are satisfied.




% or, $\mu_S > 1 - \frac{(C_\texttt{P} - C_\texttt{U}) (\beta_{\texttt{U}} (1 - (1 - \alpha) \mu_S) - \gamma) (1 - (1 - \alpha) \mu_S)}{\gamma ((1 - \alpha) L  (\beta_{\texttt{U}} (1 - (1 - \alpha) \mu_S) - \gamma) - (1 - (1 - \alpha) \mu_S) C_{\texttt{P}})}$. Thus, the above equilibrium point is obtained if and only if both $\mu_S > 1 - \frac{(C_\texttt{P} - C_\texttt{U}) (\beta_{\texttt{U}} (1 - (1 - \alpha) \mu_S) - \gamma) (1 - (1 - \alpha) \mu_S)}{\gamma ((1 - \alpha) L  (\beta_{\texttt{U}} (1 - (1 - \alpha) \mu_S) - \gamma) - (1 - (1 - \alpha) \mu_S) C_{\texttt{P}})}$ and $(1 - \alpha) L (\beta_{\texttt{U}} (1 - (1 - \alpha) \mu_S) - \gamma) > (1 - (1 - \alpha) \mu_S) C_{\texttt{P}}$ are satisfied.

 
\end{itemize}


% $y^\star = 1 - \frac{\gamma}{\betap (\alpha + (1 - \alpha) \mu_{S})}$. For notational simplicity we denote $\Delta U[\Stb] = -\epsilon$, such that $\epsilon \geq 0$. Additionally, $\frac{\gamma \epsilon - (\betap \alpha - \gamma) (C_{\Ut} - C_{\Pt})}{\betap (1 - \alpha) (C_{\Ut} - C_{\Pt} + \gamma \epsilon)} \leq 1$ should hold to ensure $\mu_{S} \leq 1$, which on simplification reduces to
% \begin{align}
%     \epsilon \leq \frac{(C_{\Ut} - C_{\Pt}) (\betap - \gamma)}{\gamma (1 - \betap (1 - \alpha))}.
%     \label{eq:epsilon}
% \end{align}

% Substitution of $\epsilon = C_{\Pt} - (1 - \alpha) L \betap y^\star(1, 0)$ in \eqref{eq:epsilon} results in the following

% \begin{align*}
%    & C_{\Pt} - (1 - \alpha) L \betap y^\star(1, 0) \leq \frac{(C_{\Ut} - C_{\Pt}) (\betap - \gamma)}{\gamma (1 - \betap (1 - \alpha))},
%    \\& \iff y^\star(1, 0) \geq \frac{C_{\Pt} \betap (1 - \gamma (1 - \alpha)) - C_{\Ut} (\betap - \gamma)}{\gamma (1 - \alpha) L \betap (1 - \betap (1 - \alpha))},
%    \\& \iff \mu_{S} \geq \frac{\gamma - \alpha \betap (1 - A)}{\betap (1 - A) (1 - \alpha)},
% \end{align*}
% where $A = \frac{C_{\Pt} \betap (1 - \gamma (1 - \alpha)) - C_{\Ut} (\betap - \gamma)}{\gamma (1 - \alpha) L \betap (1 - \betap (1 - \alpha))}$. The last step is obtained by applying the relation $y^\star(1, 0) = 1 - \frac{\gamma}{\betap (\alpha + (1 - \alpha) \mu_{S})}$.

\newpage
\um{\begin{proposition}
    First, we define some quantities of interest.
    \begin{align*}
       &\mu_{S,\mathtt{min}} (y^*_{\mathtt{i, min}}) = 1 - \frac{\yint (C_{\Ut} - C_{\Pt})}{( 1 - y^*_{\mathtt{i, min}}) (C_{\Pt} - (1 - \alpha) L \betap y^*_{\mathtt{i, min}})},
         \\&B = C_{\Pt} + (1 - \alpha) L (\betap - \gamma) + (1 - \alpha) (C_{\Ut} - C_{\Pt}),
        \\ &y^*_{\mathtt{1, min}} = \frac{B + \sqrt{B^2 - 4 (1 - \alpha) L \betap^2 (\betap - \gamma) C_{\Pt}}}{2 (1 - \alpha) L \betap^2}, 
         \\ &y^*_{\mathtt{2, min}} = \frac{B - \sqrt{B^2 - 4 (1 - \alpha) L \betap^2 (\betap - \gamma) C_{\Pt}}}{2 (1 - \alpha) L \betap^2}.
    \end{align*}
    Then, $(1 - \frac{\gamma}{\betap (\alpha + (1 - \alpha) \mu_{S})}, 1, 0)$ is a SNE if and only if 
    \begin{align*}
         & 0 < \mu_{S,\mathtt{min}} (y^*_{\mathtt{i, min}}) \leq \mu_{S} \leq \frac{\gamma - \alpha \betap (1 - \yint)}{\betap (1 - \alpha) (1 - \yint)} < 1,\;\; \textrm{and},
        \\& y^*_{\mathtt{i, min}} \leq 1 - \frac{\gamma}{\betap (\alpha + (1 - \alpha) \mu_{S})} < \yint < 1 - \frac{\gamma}{\betau} \;\; \textrm{for $\mathtt{i} \in \{1, 2\}$}.
    \end{align*} 
    \label{prop:big}
\end{proposition}
\begin{proof}
    The necessary condition of $\zsbar = 1$ is $\Delta U[\Stb] \leq 0$, or equivalently (at $\zibar = 0$),
    \begin{align*}
    & (1-\alpha) L (\beta_{\Pt} + (\beta_{\Ut} - \beta_{\Pt}) z_{\Itb}) y^\star- C_{\Pt} \leq 0
    \\ \iff & (1-\alpha) L \beta_{\Pt} y^\star- C_{\Pt} \leq 0
    \\ \iff & y^\star \leq \frac{C_{\Pt}}{(1-\alpha) L \beta_{\Pt}} = \yint.
\end{align*}
% Substituting $y^\star = 1 - \frac{\gamma}{\betap (\alpha + (1 - \alpha) \mu_{S})}$ yields
% \begin{align}
%     &(C_{\Pt} - (1 - \alpha) L \betap) (\alpha + (1 - \alpha) \mu_{S}) + \gamma (1 - \alpha) L \geq 0, \nonumber
%     \\& \implies \mu_{S} \geq \frac{\alpha (1 - \alpha) L \betap - \alpha C_{\Pt} - \gamma (1 - \alpha)L}{(1 - \alpha) (C_{\Pt} - (1 - \alpha) L \betap)}, \nonumber
%     \\&\textrm{when}\; C_{\Pt} - (1 - \alpha) L \betap > 0, \textrm{and,}
%     \\& \mu_{S} \leq \frac{\alpha (1 - \alpha) L \betap - \alpha C_{\Pt} - \gamma (1 - \alpha)L}{(1 - \alpha) (C_{\Pt} - (1 - \alpha) L \betap)}, \nonumber
%     \\&\textrm{when}\; C_{\Pt} - (1 - \alpha) L \betap < 0.
% \end{align}
Similarly, the necessary condition corresponding to $\zibar = 0$ is $\Delta U[\Itb] \geq 0$, or equivalently,
\begin{align*}
     -\pi^+[\St | \Itb] ((1- &\alpha) F[\St, \Ut] + C_{\Ut}) + C_{\Ut} - C_{\Pt} \geq 0,
    \\\iff (1 - \mu_{S}) ( 1 - &y^\star(1, 0)) (C_{\Pt} - (1 - \alpha) L \betap y^\star(1, 0)) 
    \\&\geq y^\star(1, 0) (C_{\Ut} - C_{\Pt})
    \\\iff \mu_{S} \geq 1 - &\frac{y^\star(1, 0) (C_{\Ut} - C_{\Pt})}{( 1 - y^\star(1, 0)) (C_{\Pt} - (1 - \alpha) L \betap y^\star(1, 0))},
\end{align*}
where, the second step is obtained by substituting $\pi^+[\St | \Itb]$ from \eqref{eq:pi_plus_s_ibar}. We denote $\mu_{S,\mathtt{min}} (y^\star) := 1 - \frac{y^\star(1, 0) (C_{\Ut} - C_{\Pt})}{( 1 - y^\star(1, 0)) (C_{\Pt} - (1 - \alpha) L \betap y^\star(1, 0))}$. It is easy to see for the range $y^\star(1, 0) \leq \yint$ that $\mu_{S,\mathtt{min}} (y^\star)$ is monotonically decreasing in $y^\star$, with its lowest value at $y^\star(1, 0) = \yint$, i.e., when $\mu_{S,\mathtt{min}} (y^\star) = \mu_{S,\mathtt{min}} (\yint)$. 
\\In this regime the infection state equilibrium is $y^\star = 1 - \frac{\gamma}{\betap (\alpha + (1 - \alpha) \mu_{S})} \implies \mu_{S}(y^\star) = \frac{\gamma - \alpha \betap (1 - y^\star)}{\betap (1 - \alpha) (1 - y^\star)}$. $\mu_{S}(y^\star)$ is monotonically increasing in $y^\star$, with its highest value at $\mu_{S}(\yint) = \frac{\gamma - \alpha \betap (1 - \yint)}{\betap (1 - \alpha) (1 - \yint)}$, i.e., at $y^\star = \yint$. For stability of the equilibrium point under analyses, $\mu_{S,\mathtt{min}} (y^\star) \leq \mu_{S}(y^\star)$ must hold, as $\Delta U[\Itb] \geq 0$. For stability to be guaranteed it is necessary that $y^*_{\mathtt{min}} \leq y^\star(1, 0) \leq \yint$ holds, where $y^*_{\mathtt{min}}$ is the lowest value of infection state equilibrium for which $\mu_{S,\mathtt{min}} (y^\star) \leq \mu_{S}(y^\star)$ is valid. Accordingly, we obtain the necessary condition for the range of $\mu_{S}$ to ensure stability of the equilibrium point $y^\star(0, 1)$ as $\mu_{S,\mathtt{min}} (y^*_{\mathtt{min}}) \leq \mu_{S}(y^\star) \leq \mu_{S}(\yint)$. Equating $\mu_{S,\mathtt{min}} (y^\star) = \mu_{S}(y^\star)$ yields a quadratic equation in $y^\star$ as follows
\begin{align*}
     -\betap (1 - \alpha) &(C_{\Ut} - C_{\Pt}) y^\star + \betap (1 - y^\star) (C_{\Pt} 
    \\ - (1 - \alpha) L & \betap y^\star) - \gamma (C_{\Pt} - (1 - \alpha) L \betap y^\star) = 0,
    \\ \iff y^*_{\mathtt{1, min}} &= \frac{B + \sqrt{B^2 - 4 (1 - \alpha) L (\betap - \gamma) C_{\Pt}}}{2 (1 - \alpha) L \betap} \textrm{, and,}
    \\ y^*_{\mathtt{2, min}} &= \frac{B - \sqrt{B^2 - 4 (1 - \alpha) L (\betap - \gamma) C_{\Pt}}}{2 (1 - \alpha) L \betap},
\end{align*}
where $B = C_{\Pt} + (1 - \alpha) L (\betap - \gamma) + (1 - \alpha) (C_{\Ut} - C_{\Pt})$. Clearly we have $B > 0$. The necessity of the equilibrium point to be stable is $0 < y^*_{\mathtt{i, min}} \leq \yint$, for either, or both of $\mathtt{i} \in \{1, 2\}$. In case $0 <  y^*_{\mathtt{1, min}},  y^*_{\mathtt{2, min}} \leq \yint$ holds, it implies multiple equilibria exist. In the following discussion we prove the uniqueness of the equilibrium point under analyses. Rewriting the infection state equilibrium in terms of $\yint$ yields 
\begin{align*}
    y^*_{\mathtt{1, min}} = \frac{\yint}{2} + 0.5 + D,\;\;\;y^*_{\mathtt{2, min}} = \frac{\yint}{2} + 0.5 - D,
\end{align*}
where $D = \frac{(1 - \alpha) (C_{\Ut} - C_{\Pt}) - \gamma (1 - \alpha) L + \sqrt{B^2 - 4 (1 - \alpha) L (\betap - \gamma) C_{\Pt}}}{2 (1 - \alpha) L \betap}$. First, we assume $y^*_{\mathtt{2, min}} \leq \yint \implies 0.5 \leq D + \frac{\yint}{2}$. Accordingly, $y^*_{\mathtt{1, min}} = \frac{\yint}{2} + 0.5 + D \geq 1$. Next we assume $y^*_{\mathtt{1, min}} \leq \yint \implies 0.5 \leq \frac{\yint}{2} - D$. Thereby, $y^*_{\mathtt{2, min}} = 0.5 -\frac{\yint}{2} + D \geq 1$. This proves the uniqueness of the equilibrium. $y^*_{\mathtt{min}}$ is the lowest value of infection state equilibrium in this regime, implying $y^*_{\mathtt{i, min}} \leq 1 - \frac{\gamma}{\betap (\alpha + (1 - \alpha) \mu_{S})} \leq \yint$. When $y^*_{\mathtt{i, min}} = 1 - \frac{\gamma}{\betau}$ holds, it implies $\zibar = 1$. Thus, $\yint$ must hold values strictly smaller than $1 - \frac{\gamma}{\betau}$. Thereby, we obtain the upper bound as $y^*_{\mathtt{i, min}} \leq \yint <  1 - \frac{\gamma}{\betau}$.

For sufficiency, suppose the hypothesis stated in the proposition hold true. Let $(y^\star(z^\star_{\Stb},z^\star_{\Itb}), z^\star_{\Stb},z^\star_{\Itb})$ be a SNE. We assume that $y^\star(z^\star_{\Stb},z^\star_{\Itb}) < \yint$. We compute 
\begin{align*}
    \Delta U[\Stb]& = (1-\alpha) L (\beta_{\Pt} + (\beta_{\Ut} - \beta_{\Pt}) z_{\Itb}) y^\star(z^\star_{\Stb},z^\star_{\Itb}) - C_{\Pt},
    \\&\leq (1-\alpha) L (\beta_{\Pt} + (\beta_{\Ut} - \beta_{\Pt}) z_{\Itb}) y^\star(1, z^\star_{\Itb}) - C_{\Pt} < 0
\end{align*}
exploiting increasing monotonicity of $y^\star(z^\star_{\Stb},z^\star_{\Itb})$ in $z^\star_{\Stb}$, implying $z^\star_{\Stb} = 1$. On computing $\Delta U[\Itb]$ we obtain
\begin{align}
    \Delta U [\Itb] (y^\star(1,z^\star_{\Itb}))& = \pi^+[\St | \Itb] (y^\star(1,z^\star_{\Itb})) \Delta U[\Stb](y^\star(1,z^\star_{\Itb})) \nonumber
    \\&+ (1 - \pi^+[\St | \Itb](y^\star(1,z^\star_{\Itb}))) (C_{\Ut} - C_{\Pt}),
    \label{eq:del(1, z)}
    \\\Delta U[\Itb] (y^\star(1, 0))& = \pi^+[\St | \Itb] (y^\star(1, 0)) \Delta U[\Stb](y^\star(1, 0)) \nonumber
    \\&+ (1 - \pi^+[\St | \Itb](y^\star(1, 0))) (C_{\Ut} - C_{\Pt}).
     \label{eq:del(1, 0)}
\end{align}
$\Delta U[\Itb]$  and $\pi^+[\St | \Itb]$ are expressed as functions of $y^\star(1,z^\star_{\Itb})$ and $y^\star(1, 0)$ to show their dependency on the respective infection state equilibrium. It can be verified that $0 > \Delta U[\Stb](y^\star(1,z^\star_{\Itb})) > \Delta U[\Stb](y^\star(1, 0))$. From \eqref{eq:pi_plus_s_ibar} we see that $\pi^+[\St | \Itb]$ has the opposite monotonicity as $y^\star$. Also, recall that $y^\star$ is monotonic in $z^\star_{\Itb}$. Based on these inferences, on subtracting \eqref{eq:del(1, 0)} from \eqref{eq:del(1, z)} leads to
\begin{align*}
    \Delta U &[\Itb] (y^\star(1,z^\star_{\Itb})) - \Delta U[\Itb] (y^\star(1, 0)) 
    \\&= \pi^+[\St | \Itb] (y^\star(1,z^\star_{\Itb})) \Delta U[\Stb](y^\star(1,z^\star_{\Itb})) 
    \\&- \pi^+[\St | \Itb] (y^\star(1, 0)) \Delta U[\Stb](y^\star(1, 0)) + (\pi^+[\St | \Itb](y^\star(1, 0)) 
    \\&- \pi^+[\St | \Itb](y^\star(1,z^\star_{\Itb}))) (C_{\Ut} - C_{\Pt}) > 0
\end{align*}
Now, $\Delta U[\Itb] (y^\star(1, 0)) \geq 0$ is obtained assuming the conditions in the proposition hold. Thereby, we have $\Delta U [\Itb] (y^\star(1,z^\star_{\Itb})) > 0$, which implies $z^\star_{\Itb} = 0$. This concludes our proof.
\end{proof}

\begin{remark}
    This equilibrium point is a preferred choice as the signalling scheme will have a direct control over the infection state. $y^\star = 1 - \frac{\gamma}{\betap (\alpha + (1 - \alpha) \mu_{S})}$ is a monotonically increasing function in $\mu_{S}$. In case of full information disclosure the infection level observed is $1 - \frac{\gamma}{\betap}$. With decrease in $\mu_{S}$ within this regime (i.e., with partial information) there is a fall in the value of $y^\star$. Thus, partial information plays an effective role in reducing the infection level in this regime, provided the agents possess Bayesian rationality.
\end{remark}


\begin{theorem}
    $(y^\star(1, \zidag), 1, \zidag)$ is a SNE if and only if 
    \begin{align*}
        %\mu_{S} >& \max \big\{1 - \frac{(\betau - \gamma) (C_{\Ut} - C_{\Pt})}{\gamma (C_{\Pt} - (1 - \alpha) L (\betau - \gamma))},
        %\\& \frac{\gamma - \alpha \betap (1 - \yint)}{\betap (1 - \alpha) (1 - \yint)}\big\} < 1,\;\; \textrm{and}
        &y^\star(1, \zidag) < \ymax < 1 - \frac{\gamma}{\betau} < \yint \leq \frac{\betau - \gamma}{\betap},
    \end{align*} 
    where $y^\star(1, \zidag) = 1 - \frac{\gamma}{(\betap + (\betau - \betap) \zidag) (\alpha + (1 - \alpha) (\zidag + (1 - \zidag) \mu_{S}))}$, $\ymax = \frac{C_{\Pt}}{(1-\alpha) L (\beta_{\Pt} + (\beta_{\Ut} - \beta_{\Pt}) z_{\Itb})}$, $\zidag, \mu_{S} \in (0, 1)$.%, and $\max\{ \cdot, \cdot \}$ computes the maximum of two inputs.
    \label{prop:zidag}
\end{theorem}
\begin{proof}
    From Proposition \ref{prop:unstable} it is inferred that $(y^\star(1, \zidag), 1, \zidag)$ is the \emph{only other stable SNE} that the states converge to. Characterization of the stationary Nash equilibrium points in Proposition \ref{prop:y^*_p}, \ref{prop:gamma_betau}, \ref{prop:y*_int} and \ref{prop:big} leads to our first condition for the equilibrium point as follows. From previous derivations on range of $\yint$ corresponding to characterization of each equilibrium point it can be concluded that the remaining range, i.e., $1 - \frac{\gamma}{\betau} < \yint \leq \frac{\betau - \gamma}{\betap}$ must be one of the conditions leading to this equilibrium point. The necessary condition pertaining to $\zsbar = 1$ is $\Delta U[\Stb] \leq 0$, or equivalently,
    \begin{align*}
    & (1-\alpha) L (\beta_{\Pt} + (\beta_{\Ut} - \beta_{\Pt}) z_{\Itb}) y^\star(1, \zibar) \leq C_{\Pt},
    \\ \iff & y^\star(1, \zibar) \leq \frac{C_{\Pt}}{(1-\alpha) L (\beta_{\Pt} + (\beta_{\Ut} - \beta_{\Pt}) z_{\Itb})} := \ymax.
    \end{align*}
     Clearly, $\ymax < \yint$, thereby $y^\star(1, \zibar) \leq \ymax < 1 - \frac{\gamma}{\betau} < \yint \leq \frac{\betau - \gamma}{\betap}$ holds. %Now, $0 < \zibar < 1$ must be satisfied in this range. As $y^\star$ is monotonic in $\zibar$, when $\zibar(y^\star = \ymax) < 1$ it implies $\zibar < 1$ throughout this range. For notational simplicity we introduce $\beta_{1} := \betap + (\betau - \betap) z$, and $\beta_{2} := \alpha + (1 - \alpha) (\mu_{S} + (1 - \mu_{S}) z)$, where $z := \zidag$ in this range. 
%      Similarly, the necessary condition corresponding to $\zibar \in (0, 1)$ is $\Delta U[\Itb] = 0$, or equivalently,
% \begin{align*}
%      &-\pi^+[\St | \Itb] ((1- \alpha) F[\St, \Ut] + C_{\Ut}) + C_{\Ut} - C_{\Pt} = 0,
%     \\&\iff (1 - \mu_{S}) (1 - y^\star(1, \zsdag)) ((1 - \alpha) L (\betap + (\betau - \betap) \zibar)  
%     \\&y^\star(1, \zsdag) - C_{\Pt}) = y^\star(1, \zsdag) (C_{\Pt} - C_{\Ut}),
%     \\&\iff \mu_{S} = 1 
%     \\&- \frac{y^\star(1, \zsdag) (C_{\Ut} - C_{\Pt})}{(1 - y^\star(1, \zsdag)) (C_{\Pt} - (1 - \alpha) L (\betap + (\betau - \betap) \zibar) y^\star(1, \zsdag))}
% \end{align*}
% The second step is obtained by substituting $F[\St, \Ut] = -L (\betap + (\betau - \betap) \zibar) y^\star(1, \zsdag)$, and $\pi^+[\St | \Itb]$ from \eqref{eq:pi_plus_s_ibar}. Rewriting the previous equation we obtain

For sufficiency, suppose the hypothesis stated in the proposition hold true. Let $(y^\star(z^\star_{\Stb},z^\star_{\Itb}), z^\star_{\Stb},z^\star_{\Itb})$ be a SNE. We compute 
\begin{align*}
    \Delta U[\Stb] &= (1 - \alpha) L (\betap + (\betau - \betap)\zibar) y^\star(\zsbar, \zibar) - C_{\Pt} < 0,
    \\& \implies \zsbar = 1. 
\end{align*}
% Similarly, on computing $\Delta U[\Itb]$ yields
% \begin{align*}
%     \Delta U[\Itb] &= -\pi^+[\St | \Itb] ((1- \alpha) F[\St, \Ut] + C_{\Ut}) + C_{\Ut} - C_{\Pt}.
% \end{align*}
As $1 - \frac{\gamma}{\betau} < \yint \leq \frac{\betau - \gamma}{\betap}$ holds, the conditions corresponding to Proposition \ref{prop:gamma_betau} and \ref{prop:big} are not satisfied. Thereby, $\zsbar = 1$, and $\zibar = \zidag \in (0, 1)$ are the associated fractions of susceptible and infected agents, respectively, who remain unprotected when $1 - \frac{\gamma}{\betau} < \yint \leq \frac{\betau - \gamma}{\betap}$ is true.%, and $\mu_{S} > \max\{1 - \frac{(\betau - \gamma) (C_{\Ut} - C_{\Pt})}{\gamma (C_{\Pt} - (1 - \alpha) L (\betau - \gamma))}, \frac{\gamma - \alpha \betap (1 - \yint)}{\betap (1 - \alpha) (1 - \yint)}\} < 1$ are true. 
This concludes our proof.
\end{proof}
\begin{remark}
    Similar to the case analysed in Proposition \ref{prop:big}, the infection level in this equilibrium point is monotonically increasing in $\mu_{S}$, such that the highest infection is observed at $\mu_{S} = 1$. As a result, the signalling scheme and disclosure of partial information is capable of reducing the infection level, when compared to full information disclosure.
\end{remark}
}



